Gravitational-wave extraction from neutron-star oscillations

We compare different gravitational-wave extraction methods used in three-dimensional nonlinear simulations against linear simulations of perturbations of spherical spacetimes with matter. We present results from fully general-relativistic simulations of a system composed by an oscillating and non-rotating star emitting gravitational radiation. Results about the onset of non-linear effects are also shown.

==> Makefile <==
#---------------------------------------------------------------------
#
# MAKE FILE FOR TEX COMPILER
#
#---------------------------------------------------------------------

.SUFFIXES: .tex .dvi .ps .eps .pdf

#---------------------------------------------------------------------
# Runs latex a few times, with bibtex in there too
#---------------------------------------------------------------------

.tex.dvi:
	latex $*
	latex $*
#	bibtex $*
#	latex $*
#	latex $*
#	latex $*

#---------------------------------------------------------------------
# Runs pdflatex a few times, with bibtex in there too
#---------------------------------------------------------------------

.tex.pdf: Psie20_t_pert_Times.pdf Psie20_t_pert_fit1_Times.pdf \
	Psie20_t_pert_fit2_Times.pdf PSD_Psie20_pert_1_Times.pdf \
	PSD_Psie20_pert_2_Times.pdf MaxPsie20_r_pert.pdf \
	MaxPsie20_r_pert_fit.pdf 3Dcomp1.pdf  \
	3Dcomp2.pdf A20_lambda_cmp.pdf PSD_rholm.pdf
	pdflatex $*
#	bibtex $*
#	pdflatex $*
#	pdflatex $*

#---------------------------------------------------------------------
# Produces a postscript file
#---------------------------------------------------------------------

.dvi.ps:
	dvips $* -o $*.ps

#---------------------------------------------------------------------
# Produces a pdf file
#---------------------------------------------------------------------

.ps.pdf:
	pstopdf $*.ps

#---------------------------------------------------------------------
# Produces a pdf file from an eps file
#---------------------------------------------------------------------

.eps.pdf:
	epstopdf $*.eps

all: waves_from_NS.ps

paper.dvi: waves_from_NS.tex 
paper.ps: waves_from_NS.dvi

clean:
	rm -f *.log
	rm -f *.aux
	rm -f *.dvi
	rm -f *.ps
	rm -f *.pdf
	rm -f *~

